Nearly Optimal Dynamic Set Cover: Breaking the Quadratic-in-$f$ Time Barrier

The dynamic set cover problem has been subject to extensive research since the pioneering works of [Bhattacharya et al, 2015] and [Gupta et al, 2017]. The input is a set system $(U, S)$ on a fixed collection $S$ of sets and a dynamic universe of elements, where each element appears in a most $f$ sets and the cost of each set lies in the range $[1/C, 1]$, and the goal is to efficiently maintain an approximately-minimum set cover under insertions and deletions of elements. Most previous work considers the low-frequency regime, namely $f = O(\log n)$, and this line of work has culminated with a deterministic $(1+\epsilon)f$-approximation algorithm with amortized update time $O(\frac{f^2}{\epsilon^3} + \frac{f}{\epsilon^2}\log C)$ [Bhattacharya et al, 2021]. In the high-frequency regime of $f = \Omega(\log n)$, an $O(\log n)$-approximation algorithm with amortized update time $O(f\log n)$ was given by [Gupta et al, 2017]. Interestingly, at the intersection of the two regimes, i.e., $f = \Theta(\log n)$, the state-of-the-art results coincide: approximation $\Theta(f) = \Theta(\log n)$ with amortized update time $O(f^2) = O(f \log n) = O(\log^2 n)$. Up to this date, no previous work achieved update time of $o(f^2)$. In this paper we break the $\Omega(f^2)$ update time barrier via the following results: (1) $(1+\epsilon)f$-approximation can be maintained in $O\left(\frac{f}{\epsilon^3}\log^*f + \frac{f}{\epsilon^3}\log C\right) = O_{\epsilon,C}(f \log^* f)$ expected amortized update time; our algorithm works against an adaptive adversary. (2) $(1+\epsilon)f$-approximation can be maintained deterministically in $O\left(\frac{1}{\epsilon}f\log f + \frac{f}{\epsilon^3} + \frac{f\log C}{\epsilon^2}\right) = O_{\epsilon,C}(f \log f)$ amortized update time.

==> algonew.tex <==
\section{Algorithm description}
We will describe subroutines $\del(e)$, $\ins(e)$, $\fix(e, l)$, and $\reset(k)$ which constitute the main update algorithm which is shown as \Cref{main-alg}. At the beginning of the algorithm, we assume $\univ$ is empty, and so all sets in $\set$ are initialized on level $0$. When an element $e$ is deleted from $\univ$, we will call subroutine $\del(e)$ to deal with it; if an element $e$ is inserted, then we will call $\ins(e)$. The insertion of $e$ with an appropriate intrinsic level (namely, $l = \ceil{\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon}\}} + \max_{s\ni e}\{\lev(s) \}$) might violate \Cref{inv} for some sets $s\ni e$. Hence, we apply subroutine $\fix(e, l)$ where parameter $l = \ceil{\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon}\}} + \max_{s\ni e}\{\lev(s) \}$, whose goal is to make $e$ a passive element on level $l$ and add $e$ to all the linked lists $P_l(s), \forall s\ni e$.

%Hence, we invoke $\fix(e)$ to restore \Cref{inv}(1)(2)(3) \shay{this sentence is subsumed by the following}.

% [[S: is (2) violated? (I think only as a result of $\fix(e)$ (2) might be violated)]].

%  [[S: where does this happen in the pseudo-code?]]



After that, we check if \Cref{inv}(4) is violated. If so, we find the smallest index $k$ such that $\phi_{\leq k} > \epsilon\cdot \left(c(T_{\leq k}) + f\cdot \wts(E_{\leq k}))\right)$ and then invoke subroutine $\reset(k)$;
this is repeated until \Cref{inv}(4) holds.
\begin{algorithm}
	\caption{\textsf{DynamicSetCover}}\label{main-alg}
	initialize $\lev(s) = 0, \forall s\in \set$\;
	\ForEach{element update $e$}{
		\If{$e$ is deleted}{
			$\del(e)$\;
		}\Else{
			% compute $\zlev(e)\leftarrow \max_{s\ni e} \{\lev(e) \}$\;
			% $\fix(e, \ceil{\log_{1+\epsilon}f} + \max_{s\ni e}\{\lev(s) \})$\;
			$\ins(e)$\;
		}
		\While{\Cref{inv}(4) is violated}{\label{main-while}
			find the smallest $k$ such that $\phi_{\leq k} > \epsilon\left(c(T_{\leq k}) + f\cdot \wts(E_{\leq k})\right)$\;\label{find-k}
			$\reset(k)$\;
		}
	}
\end{algorithm}

To implement \Cref{find-k} which finds the smallest index $k$ such that $\phi_{\leq k} > \epsilon\cdot \left(c(T_{\leq k}) + f\cdot \wts(E_{\leq k})\right)$, start with $k = 0$ and each time increase $k$ to the next index $k\leftarrow k^\prime$ where $T_{k^\prime}\neq \emptyset$ using the doubly linked list data structure, and check if $\phi_{\leq k} > \epsilon\cdot \left(c(T_{\leq k}) + f\cdot \wts(E_{\leq k})\right)$. In this way, the runtime of locating the smallest $k$ would be $O(|T_{\leq k}|)$ \shay{later we use a more refined bound}; note that the amount of time spent per nonempty level is constant, since we've maintained the quantities per each level separately, and we just need to sum the quantities for prefixes of levels.

%[[S: this is related to another comment below; should clarify that the amount of time spent per nonempty level is constant, since we've maintained the quantities per each level separately and we just need to sum the quantities for prefixes of levels]].

\subsection{Deletion}
We handle deletions in the same way as \cite{bhattacharya2021dynamic} which is summarized in \Cref{del}. When an element $e$ is deleted, the algorithm subtracts, for each set $s$ containing element $e$, its weight $\wts(s)$ by $\wts(e)$, and compensates for the loss by increasing the dead weight $\phi(s)$ by the weight of $e$ if $s$ was tight. This process takes  time $O(f)$.

%\anton{Can't we remove the tightness check? It seems that this doesn't affect the analysis, but makes the algorithm a bit simpler.} \tianyi{If $s$ was not tight, then $\lev(s) = 0$. Level-$0$ sets do not need to have dead weight, I suppose. It seems you are right as well.}

%{\color{red} [[A: I think it should be $\wts(s)$ here]]} 

\begin{algorithm}
	\caption{$\del(e)$}\label{del}
	\ForEach{set $s\ni e$}{
		$\wts(s)\leftarrow \wts(s) - \wts(e)$\;
		\If{$s$ was tight}{
			$\phi(s)\leftarrow \phi(s) + \wts(e)$\;
			\If{$\wts(s) + \phi(s) >c_s$}{
				$\phi(s)\leftarrow \max\{0, c_s - \wts(s) \}$\;
			}
		}
	}
\end{algorithm}

Besides, we also need to specify how to maintain the underlying data structures after an element deletion. If $e$ is active, then we go over all sets $s\ni e$ and remove $e$ from the linked list $A_{\lev(e)}(s)$; if $e$ is passive, then we go over all sets $s\ni e$ and remove $e$ from the linked list $P_{\ilev(e)}(s)$. This operation takes time $O(f)$.

As for the invariants, since $\del(e)$ does not increase any weight $\wts(s)$, \Cref{inv}(1) is preserved. Also, \Cref{inv}(2)(3) are also preserved due to the way we modify the dead weights. \Cref{inv}(4) might be violated due to increases of some dead weights, but it will be restored by the while-loop on \Cref{main-while} of \Cref{main-alg}.

% \shay{agreed; again, I suggest to omit $\zlev$ from the alg and mention something about this in the analysis only}

% \anton{$\zlev(e)$}

\subsection{Insertion}
\paragraph{High-level idea.} When inserting an element $e$, the invariants might be violated (in particular, \Cref{inv}(1) for some $s \ni e$). We try to make the newly inserted element $e$ active at level $\max_{s\ni e}\{\lev(s) \}$ if possible, and if not we try to make it passive at the lowest possible intrinsic level up to $l = \max_{s\ni e}\{\lev(s) \} + \left\lceil\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon} \}\right\rceil$; only if both these options aren't possible, we invoke $\fix(e, l)$. Thus, we invoke $\fix(e, l)$ only when we can't make the element passive at level $l \le \max_{s\ni e}\{\lev(s) \} + \log_{1+\eps} f$, which roughly speaking implies that the potential increase is very small \shay{I think it's good to provide this sentence, but we have to accompany it with some discussion on what's the meaning of potential increase} --- by a $1/f$ factor smaller compared to if we could make the element passive at level $\approx \max_{s\ni e}\{\lev(s) \}$. %\anton{Should be $l \le \max_{s\ni e}\{\lev(s) \} + \log_{1+\eps} f$, because we can always place an element at a very high level, so its weight is almost 0.}

%\anton{I find this a bit confusing, because in the algorithm, $F \neq \emptyset$ doesn't always mean that invariant \Cref{inv}(1) is violated. So actually it might be possible to make $e$ passive at level $l$, but we still invoke $\fix(e, l)$.} \tianyi{We only need a sufficient condition; that is, if $F = \emptyset$, then we can insert $e$ without applying $\fix$.}

\paragraph{Formal details.} Upon an insertion $e$, assign $\lev(e) =\max_{s\ni e}\{\lev(s) \}$. Define $l = \max_{s\ni e}\{\lev(s) \} + \left\lceil\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon} \}\right\rceil$, and define $F = \{s\ni e\mid \wts(s) + (1+\epsilon)^{-l} > c_s \}$. 
%\shay{It might be helpful to give some intuitive explanation, because I think it is key to understanding the alg.}


\begin{enumerate}[(1),leftmargin=*]
	\item If $F = \emptyset$, then compute the smallest index $h\geq \lev(e)$ such that $\wts(s) + (1+\epsilon)^{-h} \leq c_s, \forall s\ni e$. If $h = \lev(e)$, then activate $e$ on level $h$; otherwise make $e$ a passive element with intrinsic level $h$. Note that in this case, \Cref{inv}(3) is always satisfied.
	%\shay{is this equivalent to assigning $\phi(s)\leftarrow\max\{c_s - \wts(s), 0\}$? better to be consistent with the psueodo-code}.
	
	\textbf{A technical note.} To compute $h$ in $O(f)$ time, we can first compute the minimum value of the gap $c_s - \wts(s)$, and then enumerate all values $[\lev(e), l]$ to find $h$, which takes at most $O(\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon} \}) = O(f + \frac{\log C}{\epsilon}) = O(f)$ time \shay{I think the term $\frac{\log C}{\epsilon}$ should be $\frac{\log C}{\epsilon} + \frac{\log(1/\eps)}{\eps}$; also, why do we assume that these terms are subsumed in $O(f)$?}. This operation will appear again in subroutine $\reset$.
	
	%\anton{Couldn't the element become active here, if $h = \zlev(e) = \lev(e)$. Also, how do we compute $h$? It seems that we want to depend here on the number of levels. Are we using some other properties here?}
	\item If $F \neq \emptyset$, then apply subroutine $\fix(e, l)$, which will make it a passive element on level $l$ or higher, but  it will keep the gap $\ilev(e)-\lev(e)$ bounded by at most \shay{could it be smaller than this?} $\left\lceil\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon} \}\right\rceil$.
	%\anton{It will make it a passive element on level $l$ or higher. Maybe add that it will preserve the gap between $\ilev(e)$ and $\lev(e)$ by increasing $\lev(e)$ as well.}
\end{enumerate}

\begin{algorithm}
	\caption{$\ins(e)$}\label{ins}
	assign $\zlev(e) \leftarrow\max_{s\ni e}\{\lev(s) \}$\;
	Define $l \leftarrow  \max_{s\ni e}\{\lev(s) \} + \left\lceil\log_{1+\epsilon}\max\{f, \frac{2C}{\epsilon} \}\right\rceil$\;
	compute $F \leftarrow \{s\ni e\mid \wts(s) + (1+\epsilon)^{-l} > c_s \}$\;
	\If{$F = \emptyset$}{
		compute the smallest index $h\geq 0$ such that $\wts(s) + (1+\epsilon)^{-h} \leq c_s, \forall s\ni e$\;
		\If{$h>\zlev(e)$}{
			make $e$ a passive element with intrinsic level $h$\;
		}\Else{
			make $e$ an active element on level $\zlev(e)$\; %\anton{$\zlev(e)$?}
		}
		%\ForEach{$s\ni e$}{
		%	$\phi(s)\leftarrow\max\{c_s - \wts(s), 0\}$\;
		%}
	}\Else{
		$\fix(e, l)$\;
	}
\end{algorithm}

\subsection{Fixing levels}
When subroutine $\fix(e, l)$ is called, we want to assign the intrinsic level of a passive or new element $e$ to $l$, so \Cref{inv}(1) might be violated because of $e$'s update. In order to restore \Cref{inv}(1), the algorithm will repeatedly increase the level of $s$ \shay{$s$ is undefined here; I suppose we need to explain that $s$ is any set that violates \Cref{inv}(1)} until \Cref{inv}(1) is satisfied. Before describing how to implement this approach, there are two technical caveats we would like to explain.
\shay{one suggestion to clarify: ``... the algorithm will repeatedly increase the level of $s$, together with $l$, so that their gap remains the same, until \Cref{inv}(1) is satisfied}

\shay{re your suggestion: $d$ is undefined until the technical caveats below. Also, above I suggested a way to clarify, which might suffice}

\anton{I think we should change $\fix(e, l)$ a bit. This definition is a bit confusing, because in fact, it doesn't place $e$ at intrinsic level $l$, as it could place it higher. We can change it to $\fix(e, d)$, which will make the gap to be $d$. So the paragraph would be the following:

When subroutine $\fix(e, d)$ is called, we want to make the intrinsic level of $e$ to be $\lev(e) + d$, so \Cref{inv}(1) might be violated because of $e$'s update. In order to restore \Cref{inv}(1), the algorithm will repeatedly increase the level of $s$ until \Cref{inv}(1) is satisfied. Before describing how to implement this approach, there are two technical caveats we would like to explain.
}

\paragraph{Technical caveats.} When the level of $s$ increases, the level of $e$ may also increase, which decreases the gap between its intrinsic level $\ilev(e)$ and its current level $\lev(e)$. However, if $\wts(e)$ is very close to $(1+\epsilon)^{-\lev(e)}$, then for the runtime analysis, the potential function will increase by too much \shay{unclear, try to elaborate}. So, our rule here is to keep the gap $d=\ilev(e) - \zlev(e)$ unchanged by incrementing $\ilev(e)$  together with $\lev(e)$.

% \shay{this is unclear to me; what's wrong if the gap decreases?}

% \shay{when a level of $s$ rises, why would $\wts(s)$ rise? it seems that only the newly inserted element could raise $\wts(s)$; if this is the case, why not just mentioning that we want the newly inserted element to have a small enough weight, so that $\wts(s)$ doesn't violate the invariant, and to this end we increase its intrinsic level (and we stick to keeping the same gap $d$}

% \shay{if the level increases and the intrinsic level stays the same, then the gap between them decreases and the passive potential only decreases}

If we enumerate all sets $s\ni e$ in an arbitrary order, and increase $\ilev(e)$ in each round, then the tightness of some previously visited sets $s^\prime\ni e$ might be violated. To avoid this issue, in the original algorithm of \cite{bhattacharya2021dynamic}, they enumerated the sets $s\ni e$ by increasing order \shay{order of costs?}, which already takes $O(f\log f)$ time; note that one cannot use a linear-time approximate sorting algorithm, since exact sorting is needed. To circumvent the $\Omega(f \log f)$  sorting time overhead, we will make do with an arbitrary ordering of these sets, and restore tightness by increasing their dead weights \shay{unclear}.

% \shay{this is a bit risky to write, since as we mentioned one can probably apply some bucket sort to get a multiplicative error of $1+\eps$}

% \shay{should explain that $k$ denotes the levels of sets that will be enumerated by the alg}

There are two issues when $\ilev(e)$ increases.
\begin{itemize}[leftmargin=*]
	\item Each time the intrinsic level $\ilev(e)$ of $e$ changes, we may need to update the weights of sets $s^\prime\ni e$, which already takes $O(f)$ time. When $A_{\lev(s)}(s)$ is empty, we cannot charge this amount of time cost to potential loss.
	
	%\tianyi{if we naively update every change, the runtime would be high if $\ilev(e)$ changes a lot of times.} \shay{add: if we naively update every change, this will give rise to an update time of $O(f^2)$ (right?)} 
	
	To resolve this issue, we will update the contribution of $\wts(e)$ to other $\wts(s^\prime), s^\prime\in e$ in a lazy manner only when $s^\prime\ni e$ is being enumerated (which is when we actually need the updated value of $\wts(s^\prime)$).
	
	%\shay{this seems important, can you elaborate? what exactly is being deferred to a later stage, why is it important to defer it, why is clear that at a later stage it'll be handled, etc. Also, should it be numerated or enumerated?}
	
	\item The decrease of $\wts(e)$ might also violate the tightness of other sets $s\ni e$, but adding to dead weights to $\phi(s)$ due to $e$ might be too costly. In practice, we will only compensate $\phi(s)$ if $\wts(s)\geq c_s$ at the beginning of the algorithm. Otherwise, if $\wts(s) < c_s$ at beginning of the algorithm, then we can show that $s$ must be slack before $\fix(e, l)$ provided that the gap $d = \ilev(e) - \zlev(e)$ is at least $\log_{1+\epsilon}\frac{2C}{\epsilon}$; see \Cref{tight} for the actual, more general statement that we prove.
	
	%\tianyi{I have added this sentence above.}
	%\shay{Maybe: see \Cref{tight} for the actual, more general statement that we prove.}
%	We actually prove a somewhat different claim
	%	\tianyi{\Cref{tight} is more general than this. I intended to write a high-level overview, but it does not translate to formal proofs sentence by sentence.}
%	\shay{Q: do we show that?} 
	
	% \shay{unclear why does this solve the problem? details/intuition would help}
	
	% \shay{if there's a specific claim that proves that, let's refer to it here; for example, Claim 4.5 seems relevant, but it's not exactly showing this} 
\end{itemize}


\paragraph{Formal details.} Next, let us describe the algorithm more formally, which is summarized as \Cref{fix}. The algorithm assumes that $\zlev(e)$ is equal to $\lev(e)$ at the beginning. Let $\ilev^\old(e)>l$ be the intrinsic level of the element $e$ right before the execution of $\fix(e, l)$; if $e$ is a newly inserted element, then define $\ilev^\old(e) = \infty$.

%\anton{What is $\ilev^{\old}$ in case of freshly iserted item. Seems like it is not defined anywhere.}

% \shay{if this doesn't occur in the pseudo-code, I think we should either add to the psuedo-code or at least mention that (so the readers know not to look for it)}

First, assign a new intrinsic level $\ilev(e)\leftarrow l$, update all weights $\wts(s), s\ni e$, and add $e$ to $P_l(s)$ for each $s\ni e$. Keep a record $d = l - \zlev(e)$ at the beginning, and define $F = \{s\ni e\mid \wts(s)> c_s \}$.

\begin{comment}
	During the algorithm, we will make sure that the lazy level $\zlev(e)$ is always equal to $\lev(e)$, and the initial gap $\ilev(e) - \lev(e) = d$ never changes. The algorithm then goes over each set $s\ni e$ and updates the weight of $s$ according to the true $\wts(e)$;
	since $\wts(e)$ may have changed throughout the algorithm's execution, from $(1+\epsilon)^{-l}$ to some possibly lower weight,  yet we haven't updated $\wts(s)$ accordingly, the update of $s$ is done as follows:  $\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l} + \wts(e)$.
\end{comment}

%\anton{I suggest rewriting this paragraph the following way:} \tianyi{Sure.}

During the algorithm, we will make sure that the lazy level $\zlev(e)$ is always equal to $\lev(e)$, and the initial gap $\ilev(e) - \lev(e) = d$ never changes. The algorithm then goes over each set $s\ni e$ and process it the following way: First, it updates the weight of $s$ according to the true $\wts(e)$;
since $\wts(e)$ may have changed throughout the algorithm's execution, from $(1+\epsilon)^{-l}$ to some possibly lower weight,  yet we haven't updated $\wts(s)$ accordingly, the update of $s$ is done as follows:  $\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l} + \wts(e)$.

After that, whenever $\wts(s, \lev(s)+1) \geq c_s$, we can first zero out its dead weight $\phi(s)\leftarrow 0$ according to \Cref{inv}(3), and then we increase the level of $s$ by $1$; recall that $\wts(s, \lev(s)+1)$ can be computed in constant time given $\wts(s), |A_{\lev(s)}(s)|$. In each iteration of the while-loop, the algorithm does the following steps.

%\anton{This increase is not reflected in the pseudocode. And I suggest leaving that increase where it used to be (at line 24, which is still in the pseudocode). Also, this doesn't remove the need to analyze the case of $s$, since we still can gain some dead weight during the foreach in line 14. But in that case we can argue that the down potential increase is not big. See my comment and the proposed fix in the runtime section.} \tianyi{Sure, I will switch to your version.}

% \anton{How do we recalculate or maintain $\wts(s, \lev(s) + 1)$?}

% \anton{I don't understand what this means. It seems like we set $\wts(e)$ to $(1 + \epsilon)^{-l}$, so we modify $\wts(s)$ accordingly. But in some sense it undoes all the previous modifications. Also, do we even need this, since in the first line we did this anyway?} \shay{This is indeed unclear}

% \shay{in general, it's better to avoid ``update''; I'd change to update/set/reset (here and elsewhere)}
\begin{enumerate}[(1),leftmargin=*]
	\item Define $k = \lev(s)$. First, consider the case where $k<\bs(s)$. If $\zlev(e) <\bs(s)$ and $\bs(s) + d > \ilev^\old(e)$, then simply put $\zlev(e), \lev(s) \leftarrow \ilev^\old(e) - d$, $\ilev(e)\leftarrow\ilev^\old(e)$ and quit the while-loop. 
We will prove that $\wts(s, \lev(s) + 1) < c_{s}$ holds after the update, and so we can safely quit the while loop.
	
%	\shay{actually, I think we should explain why this holds (I think the answer is in the proof of Claim 4.1, i.e., you can't have any elements lower than the base, but the readers haven't reached yet Claim 4.1 so they don't know..)}, 
	
	%\anton{But before this at the begining we made $e$ a passive element with $\ilev(e)$ and added it to $P_{l}(s)$. Perhaps, we should add some procedure Setilev, which takes care of all the sets.} \shay{indeed we need to remove $e$ from $P_l(s)$ and add it back to the old list}
	%\anton{I think we need to explain here why after that $\wts(s, \lev(s) + 1) < c_{s}$, so we can quit the loop.}
	%\shay{perhaps it suffices to write that: after the update we have $\wts(s, \lev(s) + 1) < c_{s}$, and we can safely quit the while loop}
	
	Otherwise, assign $\lev(s) \leftarrow \bs(s)$. If $\zlev(e) = \lev(e)$ should now increase to $\bs(s)$, assign $\ilev(e)\leftarrow \bs(s)+d$. Then, we need to activate all passive elements in $P_{\lev(s)}(s)\setminus \{e\}$: if $P_{\lev(s)}(s)\setminus \{e\}$ is nonempty, then turn all elements in $P_{\lev(s)}(s)\setminus \{e\}$ active; that is, for each $e^\prime\in P_{\lev(s)}(s)\setminus \{e\}$, remove it from $P_{\lev(s)}(s)$ and add it to $A_{\lev(s)}(s)$. After that, continue to the next iteration.
	
	
	\item If $A_k(s)\neq\emptyset$, go over all elements $e^\prime\in A_{k}(s)$ and increase their levels $\lev(e^\prime)$ to $k+1$ as well. Because of this, for each such element $e^\prime$, we also need to go over all sets $s^\prime\ni e^\prime$ and update the value of $\wts(s^\prime)$ by a decrease of $\epsilon(1+\epsilon)^{-k-1}$.
	
	After that, for each $s^\prime\ni e^\prime, s^\prime\neq s$, to restore tightness on set $s^\prime\ni e^\prime$, we need to increase its dead weight $\phi(s^\prime)$ by $\epsilon(1+\epsilon)^{-k-1}$. Next, for each such $s^\prime$, consider two cases depending on if $e\in s^\prime$; note that membership testing can be done in $O(1)$ time after an $O(f)$-time preprocessing on all sets $s\ni e$.
	%\anton{Can we do it in $O(1)$ deterministic time?}
%		\begin{note}{A}
%		  \color{red}
%		  Can we do it in $O(1)$ deterministic time?
%		\end{note}
	\begin{enumerate}[(a),leftmargin=*]
		\item If $e\notin s^\prime$ and $\wts^*(s^\prime)$ now becomes larger than $c_{s^\prime}$, reassign $\phi(s^\prime)\leftarrow\max\{0, c_{s^\prime} - \wts(s^\prime)\}$ to restore \Cref{inv}(3).
		
		\item If $e\in s^\prime\neq s$, then since we are being lazy on updating the contribution of $\wts(e)$ to $\wts(s^\prime)$,  we do not zero out $\phi(s^\prime)$ for now. 
		
		Note that the true value of $\wts(s^\prime)$ could possibly be smaller than the value currently maintained by the algorithm, as the intrinsic level of $e$ is rising throughout the execution of the algorithm, meaning that the true weight of $\wts(e)$ decreases, yet we haven't made sure to update $\wts(s^\prime)$ accordingly. Whenever we will need the updated value of $\wts(s^\prime)$, we will make sure to ``refresh'' the up-to-date weight contribution of $\wts(e)$.

		Therefore, although \Cref{inv}(3) might be violated by $s^\prime$ for now, we will fix it in the end by assigning $\phi(s^\prime)\leftarrow \{c_s -\wts(s^\prime),0\}$ if $\wts^*(s^\prime) > c_{s^\prime}$.
		
%		\shay{in lines 34-35}
		
%		\shay{Q: in line 5, we are updating the weights. I don't understand the meaning of this update, but we're doing something there, so it's %rema bit strange to say that we're lazy} 
		
		%\shay{this item seems important, but details/intuition are missing}
	\end{enumerate}	
	
	%Similarly, to restore tightness for set $s\ni e$, if $s$ was a tight set just now, we need to increase its dead weight $\phi(s)$ by $(1+\epsilon)^{-l} - (1+\epsilon)^{-\ilev(e)}$; if $\wts^*(s)$ now becomes larger than $c_{s}$, reassign $\phi(s)\leftarrow\max\{0, c_{s} - \wts(s)\}$.
	
	Here, during the execution of $\fix$, we do not assume $s^\prime$ was tight whenever $\lev(s^\prime) > 0$. This is because $\fix$ might also be called within another subroutine $\reset$ where \Cref{inv}(2) has not been recovered.
	
	\item Now, increase $\lev(s)$ to $k+1$. If $\zlev(e) = k$, then increase $\ilev(e)$ by one and update $\wts(s)$ accordingly.
	
	Finally, activate all passive elements in $P_{\lev(s)}(s)\setminus \{e\}$: if $P_{\lev(s)}(s)\setminus \{e\}$ is nonempty, then turn all elements in $P_{\lev(s)}(s)\setminus \{e\}$ active; that is, for each $e^\prime\in P_{\lev(s)}(s)\setminus \{e\}$, remove it from $P_{\lev(s)}(s)$ and add it to $A_{\lev(s)}(s)$.
	\begin{comment}
		Next, if $\lev(e) = k$, then increase the intrinsic level $\ilev(e)$ of $e$ by one. If $b = 1$, continue to the next iteration.
		
		Otherwise, if $b=2$, update $\wts(s)$ by a decrease of $\epsilon(1+\epsilon)^{-\ilev(e)-1}$. Again, for each $s^\prime\ni e$, if $s^\prime\neq s$ and was a tight set before we decrease the weight $\wts(s^\prime)$, we need to increase its dead weight $\phi(s^\prime)$ by $\epsilon(1+\epsilon)^{-\ilev(e)-1}$; if $\wts^*(s^\prime)$ now becomes larger than $c_{s^\prime}$, reassign $\phi(s^\prime)\leftarrow\max\{0, c_{s^\prime} - \wts(s^\prime)\}$.
	\end{comment}
\end{enumerate}

\begin{comment}
	When the while-loop terminates, it keeps a record of the current value of $l_s\leftarrow \ilev(e)$ for each $s\ni e$. When all sets in $s\ni e$ have been enumerated, update the weight $\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l_s} + \wts(e)$, and restore tightness for set $s\ni e$: if $s\in F$, increase its dead weight $\phi(s)$ by $(1+\epsilon)^{-l_s} -\wts(e)$; next, if $\wts^*(s)$ is larger than $c_{s}$, reassign $\phi(s)\leftarrow\max\{0, c_{s} - \wts(s)\}$ to restore \Cref{inv}(3).
\end{comment}

%\anton{I suggest the following rewrite:} \tianyi{Sure.}

After the while-loop terminates, the algorithm keeps a record of the current value of $l_s\leftarrow \ilev(e)$ for the current set $s$. 

After all sets in $s\ni e$ have been enumerated, go over all sets $s \ni e$ again to update the weight $\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l_s} + \wts(e)$, and restore tightness for set $s\ni e$ the following way: if $s\in F$, increase its dead weight $\phi(s)$ by $(1+\epsilon)^{-l_s} -\wts(e)$; next, if $\wts^*(s)$ is larger than $c_{s}$, reassign $\phi(s)\leftarrow\max\{0, c_{s} - \wts(s)\}$ to restore \Cref{inv}(3).
%\shay{here too some intuition/details are missing}

%\anton{Maybe state ``for each s'' explicitly. Because it made me think whether it is just an auxilary value that gets reassigned each iteration, or it is a list, even though it has a subsrcipt}

\begin{algorithm}
	\caption{$\fix(e, l)$}\label{fix}
	make $e$ a passive element with $\ilev(e)\leftarrow l$, update all weights $\wts(s), s\ni e$, and add $e$ to $P_l(s)$\;
	$F \leftarrow \{s\ni e\mid \wts(s)> c_s \}$\;
	$d\leftarrow \ilev(e) - \zlev(e)$\;
	\ForEach{$s\ni e$}{
		update the weight $\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l} + \wts(e)$\; \tcp{refresh $\wts(s)$ according to up-to-date $\wts(e)$}
		\While{$\wts(s, \lev(s)+1) \geq c_s$}{\label{fix-while}
			$\phi(s)\leftarrow 0$, $k\leftarrow \lev(s)$\;
			\If{$k <\bs(s)$}{
				\If{$\zlev(e) <\bs(s)$ and $\bs(s) + d > \ilev^\old(e)$}{
					assign $\zlev(e), \lev(s) \leftarrow \ilev^\old(e) - d$, $\ilev(e)\leftarrow\ilev^\old(e)$\;
					\textbf{break}\;
				}
				$\lev(s)\leftarrow \bs(s)$ and update $\zlev(e), \lev(e)$ accordingly\;
				\If{$\zlev(e) = \bs(s)$}{
					$\ilev(e)\leftarrow \bs(s) + d$\;
				}
				%\anton{Isn't this if redundant, since we have $\ilev(e) = \zlev(e) + d$?}
				%  \anton{$\zlev(e)$?}
				activate all passive elements in $P_{\lev(s)}(s)\setminus \{e\}$\;
				\textbf{continue}\;
			}
			\ForEach{$e^\prime\in A_k(s)$}{
					$\lev(e^\prime)\leftarrow k+1$\;					
					\ForEach{$s^\prime\ni e^\prime$}{
						$\wts(s^\prime)\leftarrow \wts(s^\prime) - \epsilon(1+\epsilon)^{-k-1}$\;
						$\phi(s^\prime)\leftarrow \phi(s^\prime) + \epsilon(1+\epsilon)^{-k-1}$\;
						\If{$\wts(s^\prime) + \phi(s^\prime) > 	c_{s^\prime}$ and $e\notin s^\prime$}{
							$\phi(s^\prime)\leftarrow \max\{0, c_{s^\prime} - \wts(s^\prime)\}$\;
						}
					}
			}
			$\lev(s)\leftarrow k+1$\;
			activate all passive elements in $P_{\lev(s)}(s)\setminus \{e\}$\;
			\If{$\zlev(e) = k$}{
				% \anton{$\zlev(e)$?}
				update $\zlev(e)\leftarrow\lev(s), \ilev(e)\leftarrow \lev(s) + d$\; %\anton{Should change $\lev(e)$ to $\lev(s)$ in the first assignment.}
				$\wts(s)\leftarrow \wts(s) - \epsilon(1+\epsilon)^{-k-1-d}$\;
				%  \anton{$\lev(s)$?}
			}
			%\anton{Isn't this if redundant either, since we have $\ilev(e) = \zlev(e) + d$? It makes sense for me, if we change the condition to $\zlev(e) = k$. Because before we assigned $\lev(s) \leftarrow k + 1$, we had $\zlev(e) \leq k$, so there is a problem only when $\zlev(e) = k$.}
		}
		$l_s\leftarrow \ilev(e)$\;
	}
	\ForEach{$s \ni e$}{
		$\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l_s} + \wts(e)$\; \tcp{refresh $\wts(s)$ according to up-to-date $\wts(e)$}
		\If{$s\in F$}{
			$\phi(s)\leftarrow \phi(s) +(1+\epsilon)^{-l_s} - \wts(e)$\;
		}
		\If{$\wts(s) + \phi(s) > 	c_{s}$}{
			$\phi(s)\leftarrow \max\{0, c_{s} - \wts(s)\}$\;
		}
	}
	\begin{comment}
		\ForEach{$s \ni e$}{
			$\wts(s)\leftarrow \wts(s) - (1+\epsilon)^{-l} + (1+\epsilon)^{-\ilev(e)}$\;
			\If{$s$ was tight}{
				$\phi(s)\leftarrow \phi(s) + (1+\epsilon)^{-l} - (1+\epsilon)^{-\ilev(e)}$\;
				\If{$\wts(s) + \phi(s) > 	c_{s}$}{
					$\phi(s)\leftarrow \max\{0, c_{s} - \wts(s)\}$\;
				}
			}
		}
	\end{comment}
\end{algorithm}

\begin{figure}
	\centering
	\input{figs/fixlevel-fig}
	\caption{This picture illustrates one iteration of the while-loop that raises set $s$ during the execution of $\fix(e, l)$. There are three active elements $\{e_1, e_5, e_6\}$ denoted by black circles, four passive elements $\{e, e_2, e_3, e_4\}$ denoted by white circles. The rectangle denotes $\zlev(e)$, which is equal to $\lev(e)$. Also, there are three sets: $s = \{e, e_1, e_2, e_3, e_4, e_5\}$ denoted by red color, $s_1 = \{e_1, e_2\}$ denoted by green color, and $s_2 = \{e, e_3, e_4, e_5, e_6\}$ denoted by blue color. The level of all three sets is $k$. The left side of the picture shows the state right before the iteration, and the right side shows the state right after it. During that iteration, $e_1$ and $e_5$ got raised from level $k$ to level $k + 1$ and remain active. Elements $e_2$ and $e_4$ become active, since they were passive elements at level $k + 1$ and belong to $s$. Since the lazy level of $e$ was $k$, both lazy and intrinsic levels got raised by one, so the gap remains equal to $d$. Finally, the level of $s$ raised to $k + 1$.}
	\label{fixlevel-fig}
\end{figure}

\subsection{Rebuilding}
A rebuild operation is invoked when \Cref{inv}(4) is violated at some point. Let $k$ be the smallest index such that $\phi_{\leq k} > \epsilon\left(c(T_{\leq k}) + f\cdot \wts(E_{\leq k})\right)$; such index $k$ can be found in time:
$$O\left(\frac{\log C}{\epsilon} + |T_{\leq \ceil{\log_{1+\epsilon}C}+1}| + |E_{\leq k}|\right)$$ 
using the linked list data structure.

\anton{I think it should be $T_{\leq k} \setminus T_{\leq \ceil{\log_{1+\epsilon}C}+1}$ instead of $T_{\leq \ceil{\log_{1+\epsilon}C}+1}$}

%\anton{There used to be a paragraph entitled ``Technical caveats'', but now it's gone. Perhaps we should delete this sentence or return this paragraph. Also, I think it's better to move the paragraph about the implicit zeroing before the definition.}

%\tianyi{I have removed the sentence. I think it is more standard to put basic operations in the preliminary section.}

\begin{comment}

\paragraph{Technical caveats.} At the beginning, we need to move all sets on levels $\leq k$ to level $k+1$, and remove all the dead weights. However, even this step would be too costly since the total number of sets could be as large as $O(f|E_{\leq k}|)$. For a runtime faster than $O(f\log f)$, although we can spend $O(1)$ time for each tight set in $T_{\leq k}$, we cannot spend $O(1)$ time for each set on level-$0$. To fix this issue, the idea is that we touch those sets on level-$0$ only when necessary. Basically, these sets will be all the ones that contain active elements that were in $A_{\leq k}$ or passive elements that are to be activated on level $k+1$.
	More specifically, prepare a set $S\subseteq \set$ (initially empty) which will collect all the necessary sets on levels $\leq k$ for rebuilding. Then, go over all active elements $e\in A_{\leq k}$, and enumerate all sets $s\ni e$ on level $\leq k$ and move it to level $k+1$. Also, go over all passive elements $e\in E_{\leq k}\setminus A_{\leq k}$ and see if its intrinsic level is at most $k+1$; if $\ilev(e)\leq k+1$, then we can activate $e$ and move it to $A_{k+1}$. 
\end{comment}


\begin{definition}
	An element $e\in E_{\leq k}$ is called \emph{dirty}, if $e$ is passive and $\ilev(e) > k+1$ \shay{is it $k$? I think not (since the rebuild will change ilev to $k+1$)}; otherwise, $e$ is called \emph{clean}.
\end{definition}

% \shay{$U$ reads similarly to $\mathcal{S}$, perhaps should change letter?}

Apply implicit zeroing (check its definition in  \Cref{implicit-zeroing}) on all levels in $[0,\min\{ \ceil{\log_{1+\epsilon}C}+1, k\}]$. Then, define $U\leftarrow T_{\leq k}\setminus T_{\leq \ceil{\log_{1+\epsilon}C}+1}$, and go over all $s\in U$ and increase their levels to $k+1$, and assign $\phi(s)\leftarrow 0$.

Let us first process all clean elements in the following way (which is omitted in the pseudocode). For each clean element $e$, go over all sets $s\ni e$ on level-$0$, assign $\lev(s)\leftarrow k+1, \phi(s)\leftarrow 0$, \anton{I think we don't need to set $\phi(s)\leftarrow 0$, since this is handled by the implicit zeroing.} and add $e$ to $A_{k+1}$ (if $e$ was passive, then activate it now), and assign a new weight $\wts(e)\leftarrow (1+\epsilon)^{-k-1}$, and update all $\wts(s), \forall s\ni e$ accordingly. After that, add all such $s\ni e$ to $U$.

%\anton{This if is redundant. I think we can remove it, since the definition is nearby. And anyway, this if looks a bit strange, because it looks like we are checking something, but that's just the definition of a clean element.}

%\anton{I think we should remove ``itemize'', since there is only one item.}


% \shay{the following isn't in the pseudo-code, should at least comment about it somehow}

For the rest, we will deal with all dirty elements. Let $D$ be the set that collects all dirty elements, and define a set $\widehat{E}$ which contains all the clean elements initially. Go over each element $e\in D$. There are two different ways to process element $e$, depending on whether our algorithm uses randomization. See \Cref{reset-fig} for an illustration, and the entire $\reset(*)$ procedure is summarized as \Cref{rand-reset}.


\begin{figure}
	\centering
	\input{figs/reset-fig}
	\caption{In this picture, $\{e_1, e_2, e_3\}$ are dirty elements, and $\{e_4, e_5, e_6, e_7, e_8\}$ are clean elements which are put on level $k+1$. The $\reset(k)$ procedure tries to reduce the gaps $\ilev(e_i) - \zlev(e_i), \forall i\in \{1, 2, 3\}$. In the deterministic algorithm, the gaps decrease by at least one; in the randomized algorithm, the gaps decrease exponentially.}
	\label{reset-fig}
\end{figure}

%Note that, for dirty elements $e\in D$, although some sets $s\ni e$ might have already changed its level to $k+1$, we have not yet kept track of it and updated $\lev(e)\leftarrow k+1$. So currently the values of $\lev(e)$ in our data structure are \emph{invalid} for $e\in D$.

\paragraph{Deterministic algorithm.} First, raise all sets $s\ni e$ to level $\max\{\lev(s), k+1\}$, and add $s$ to $U$ if $\lev(s) = k+1$. If $e$ is not currently contained in any tight set, then go over all sets $s\ni e$ currently on level $k+1$ and add them to $U$, and assign $\zlev(e)\leftarrow k+1$. Then, compute $h\in [k+1, \ilev(e)]$ to be the smallest integer such that $\wts(s) - \wts(e) + (1+\epsilon)^{-h} \leq c_s, \forall s\ni e$. Note that such index $h$ must exist, since if we take $h = \ilev(e)$, all sets $s\ni e$ are currently slack and thus $\wts(s) < c_s / (1+\epsilon)$.
	
	%\shay{explain why such $h$   exists}
	
	If $h >k+1$, then assign $\ilev(e)\leftarrow h$ and update all the linked lists $P_{\ilev(e)}(s), \forall s\ni e$ accordingly. Otherwise, activate $e$ on level $k+1$ and add it to $A_{k+1}(s), \forall s\ni e$. After that, add $e$ to $\widehat{E}$.
	
	%\shay{I stopped reading here}
	\paragraph{Randomized algorithm.} We first check if $e$ is still passive. This is necessary since $e$ might have been activated when processing previous elements in $D$. If passive, then move on to the following steps.
	
	Find the index $\eta$ such that:\footnote{Recall that $\clog^{(\eta)}$ is $\clog$ iterated for $\eta$ times.} %\anton{Can we compute logarithm in $O(1)$ time? If no, maybe we should compute all $\log_{1+\epsilon}^{i}f$ beforehand.}
	$$\clog_{1+\epsilon}^{(\eta+1)}f\leq \ilev(e) - k-1\leq \clog_{1+\epsilon}^{(\eta)}f$$
	We will prove later that $\eta$ is always at least $1$. Next, define:
	$$\delta = \min\left\{\left(\frac{1}{\clog^{(\eta)}_{1+\epsilon}f}\right)^4, \brac{\frac{\epsilon}{2C}}^2\right\}\cdot (1+\epsilon)^{-k-1}$$ 
	Repeatedly take uniformly random samples of sets $s\ni e$ for $50\ceil{\frac{f}{\clog_{1+\epsilon}^{(\eta)}f}}$ times, and check if $\wts(s) -\wts(e) +\delta > c_s$. If there is one such set $s$, then we claim that $s$ is tight. To update the lazy level of $e$, first raise the set level $\lev(s)\leftarrow \max\{k+1, \lev(s)\}$, and assign $\zlev(e)\leftarrow \lev(s)$. After that, continue on to the next element $e\in D$.
	
	Otherwise, go over all sets $s\ni e$, raise them to level $\max\{k+1, \lev(e)\}$, and add them to $U$ if it is slack, and update $\zlev(e)\leftarrow \max_{s\ni e}\{\lev(s) \}$. In the meantime, compute the set $\widehat{F}$ of all $s\ni e$ such that $\wts(s) - \wts(e) + \delta > c_s$. There are three cases below.
	\begin{enumerate}[(1),leftmargin=*]
		\item $|\widehat{F}| > \left(\clog_{1+\epsilon}^{(\eta)}f\right)^2$.
		
		In this case, let us continue on to the next element $e\in D$.
		
		\item $\widehat{F} = \emptyset$.
		
		In this case, compute $$h\in \left[k+1, \min\left\{\ilev(e), \ceil{\log_{1+\epsilon}\frac{1}{\delta}}\right\}\right]$$
		which is the smallest index such that $\wts(s) - \wts(e) + (1+\epsilon)^{-h}\leq c_s, \forall s\ni e$.
		
		%\tianyi{Variable $h$ was used before. Need to use another variable name.}
		
		If $h >k+1$, then assign $\ilev(e)\leftarrow h$ and update all the linked lists $P_{\ilev(e)}(s), \forall s\ni e$ accordingly. Otherwise, activate $e$ on level $k+1$ and add it to $A_{k+1}(s), \forall s\ni e$. After that, add $e$ to $\widehat{E}$.
		
		Finally, to restore \Cref{inv}(3), for each $s\ni e$ such that $\wts(s) + \phi(s) > c_s$, assign $\phi(s) \leftarrow c_s - \wts(s)$.
		
		\item $0<|\widehat{F}| \leq \left(\clog_{1+\epsilon}^{(\eta)}f\right)^2$.
		
		In this case, we will apply subroutine $\fix$ on $e$. More specifically, invoke the  subroutine $\fix(e, \min\{\ilev(e), \zlev(e) +d\})$, where:
		$$d = \left\lceil\log_{1+\epsilon}\max\left\{\left(\clog^{(\eta)}_{1+\epsilon}f\right)^4, \brac{\frac{2C}{\epsilon}}^2\right\}\right\rceil$$
		
		As a clarification, during the $\reset(k)$ subroutine, some active elements were raised to level $k + 1$, and the sets that contain them are temporarily in an incorrect state. But because when processing $e$ we also raise every $s \ni e$, everything is still fine and subroutine $\fix$ can function correctly.
		
		%\anton{It might be helpful to add some clarification why it is okay to invoke $\fix$ here. Because during the preprocessing, some active elements were raised to level $k + 1$, and the sets that contain them are temporarily in an incorrect state. But because when processing $e$ we also raise every $s \ni e$, everything is fine. But it is not crucial, I think.}
	\end{enumerate}

\paragraph{Post-processing.} After we have processed $D$, some levels of elements in $\widehat{E}$ might be larger than $k+1$ because of $\fix$. As a post-processing step, remove all elements in $\widehat{E}$ whose levels are larger than $k+1$. Next, let $\widehat{U}\subseteq U$ be all the slack sets in $U$. For the rest, we need to use the following subroutine $\water$ from \cite{bhattacharya2021dynamic,bhattacharya2019deterministically}.

\begin{lemma}[\cite{bhattacharya2021dynamic,bhattacharya2019deterministically}]\label{waterfill}
	There is a deterministic subroutine $\water(\widehat{k}, \widehat{U}, \widehat{E})$ which takes as input a collection of sets and active elements $\widehat{U}, \widehat{E}$ on level $\widehat{k}$, such that for each $s\in \widehat{U}$, we have $\wts(s)<c_s, \phi(s) = 0$. In the end, all elements in $\widehat{E}$ are still active, and the subroutine places each set $s\in \widehat{U}$ at level $\lev(s)$ such that (1) $\wts(s) < c_s, \phi(s) = 0$, and (2) if $\lev(s) > 0$ then $\wts(s) > \frac{c_s}{1+\epsilon}$. The runtime is $O(f|\widehat{E}| +\widehat{k})$.
\end{lemma}

We cannot directly apply $\water(k+1, \widehat{U}, \widehat{E})$ since the runtime would depend on $k$. Instead, we follow the idea from \cite{bhattacharya2021dynamic} and move all elements and sets in $\widehat{E}, \widehat{U}$ to level $\widehat{k} = \min\left\{k+1, \ceil{\log_{1+\epsilon}\frac{2C\cdot|\widehat{E}|}{\epsilon}}\right\}$. The following lemma claims that directly moving elements and sets to level $\widehat{k}$ does not create weights larger than $c_s$. So in the final step, we can safely invoke $\water(\widehat{k}, \widehat{U}, \widehat{E})$. 

\begin{lemma}[\cite{bhattacharya2021dynamic}]
	After moving sets and elements in $\widehat{U},\widehat{E}$ to level $\widehat{k}$, each set $s\in \widehat{U}$ has weight less than $c_s$.
\end{lemma}


\begin{algorithm}
	\caption{$\reset(k)$}\label{rand-reset}
	apply implicit zeroing for all levels $0\leq i\leq \min\{\ceil{\log_{1+\epsilon}C}+1, k\}$\;
	define $U\leftarrow T_{\leq k}\setminus T_{\leq \ceil{\log_{1+\epsilon}C}+1}$, and assign $\phi(s)\leftarrow 0, \lev(s)\leftarrow k+1, \forall s\in U$\;
	process all clean elements\;\label{clean}
	let $D$ be the set of all dirty elements, and $\widehat{E}$ be all clean elements\;
	\ForEach{$e\in D$ which is still passive}{
		\If{deterministic}{
			assign $\lev(s)\leftarrow \max\{\lev(s), k+1\}$ and add $s$ to $U$ if $\lev(s) = k+1$, $\forall s\ni e$\;
			\If{all sets $s\ni e$ are slack}{
				compute the smallest index $h\geq k+1$ such that $\wts(s) - \wts(e) + (1+\epsilon)^{-h}\leq c_s$\;
				\If{$h>k+1$}{
					assign $\ilev(e)\leftarrow h$\;
				}\Else{
					activate $e$ on level $k+1$, and add it to $\widehat{E}$\;
				}
			}
		}
		\If{randomized}{
			find index $\eta$ such that $\clog_{1+\epsilon}^{(\eta+1)}f\leq \ilev(e) - k-1\leq \clog_{1+\epsilon}^{(\eta)}f$\;
			define $\delta \leftarrow \min\left\{\left(\frac{1}{\clog^{(\eta)}_{1+\epsilon}f}\right)^4, \brac{\frac{\epsilon}{2C}}^2\right\}\cdot (1+\epsilon)^{-k-1}$\;
			$\text{flag}\leftarrow \mathbf{true}$\;
			\For{$50\ceil{f / \clog_{1+\epsilon}^{(\eta)}f}$ times}{
				uniformly sample $s\ni e$\;
				\If{$\wts(s) - \wts(e) + \delta > c_s$}{
					assign $\lev(s)\leftarrow \max\{k+1, \lev(s)\}$, $\zlev(e)\leftarrow \lev(s)$\;
					$\text{flag}\leftarrow \mathbf{false}$ and \textbf{break}\;
				}
			}
			\If{$\text{flag}$}{\label{true-flag}
				raise all $s\ni e$ to level $\max\{\lev(s), k+1 \}$ and add them to $U$ if slack, and update $\zlev(e)\leftarrow \max_{s\ni e}\{\lev(s)\}$\;
				compute $\widehat{F} = \{s\ni e\mid \wts(s) - \wts(e) + \delta > c_s \}$\;
				\If{$\widehat{F} = \emptyset$}{\label{empty-F}
					compute the smallest index $h\geq k+1$ such that $\wts(s) - \wts(e) + (1+\epsilon)^{-h}\leq c_s, \forall s\ni e$\;
					\If{$h>k+1$}{
						assign $\ilev(e)\leftarrow h$\;
					}\Else{
						activate $e$ on level $k+1$, and add it to $\widehat{E}$\;
					}
					\ForEach{$s\ni e$}{
						$\phi(s)\leftarrow \max\{c_s - \wts(s), 0\}$\;
					}
				}\ElseIf{$|\widehat{F}| \leq \left(\clog_{1+\epsilon}^{(\eta)}f\right)^2$}{\label{small-F}
					$d \leftarrow \left\lceil\log_{1+\epsilon}\max\left\{\left(\clog^{(\eta)}_{1+\epsilon}f\right)^4, \brac{\frac{2C}{\epsilon}}^2\right\}\right\rceil$\;
					$\fix(e, \min\{\ilev(e), \zlev(e) + d\})$\;
				}
			}
		}
	}
	remove all elements in $\widehat{E}$ whose levels are $>k+1$\;
	let $\widehat{U}$ be all the slack sets in $U$\;
	$\widehat{k} = \min\left\{k+1, \ceil{\log_{1+\epsilon}\frac{2C\cdot|\widehat{E}|}{\epsilon}}\right\}$\;
	move all elements and sets in $\widehat{E}, \widehat{U}$ to level $\widehat{k}$\;
	$\water(\widehat{k}, \widehat{U}, \widehat{E})$\;
\end{algorithm}


